Weather of the Dorm WIFI Ecosystem at the University of Colorado Boulder for Fall Semester 2019 to Spring Semester 2020 a Case Study of WIFI and a Campus Response to the COVID-19 Perturbation

Growing use of network technology in Higher Education means that there has been increasing demand to adapt technology platforms and tools that transform student learning strategies, faculty teaching, research modalities, as well as general operations. Many of the new modalities are necessary for IHE business. In August 2019, we began collecting and analyzing data from the campus WIFI network. A goal of the research was to answer question like what passive sensing of the IHE WIFI might tell us about the dynamics of the WIFI weather in the IHE ecosystem and what does anonymized data tell us about the IHE ecosystem. The analogy with weather prediction seemed appropriate and a viable approach. Starting Fall 2019, data were collected in the observational phase. In the analysis phase, we applied Singular Spectrum Analysis decomposition, to deconstruct WIFI data from dorms, the central campus dining cafeteria, the recreation center, and other buildings on campus. That analysis led to the identification of clusters of buildings that behaved similarly. Just as in the case of models of the weather, a final component of this research was forecasting. We found that weekly forecast of WIFI behavior in the Fall 2019, were straight forward using SSA and seemed to present behavior of a low dimensional dynamical system. However, in Spring 2020, and the COVID perturbation, the campus ecosystem received a shock and data show that the campus changed very quickly. We found that as the campus moved to conduct remote learning, teaching, the closure of research labs, and the edict to work remotely, SSA forecasting techniques not trained on the Spring 2020, data after the shock, performed poorly. While SSA forecasting trained on a portion of the data did better.

==> references_frrom.tex <==
\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to {\LaTeX}}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.


\bibitem{Broomhead}
D. S. Broomhead and G. P. King. \textit{Extracting Qualitative dynamics from Experimental data, Physics D, 20~(1986), pp. 217--236.}

\bibitem{ Champions_2012}

Champions, K, Lusch, , Kutz,  J. N., and Brunton, S. L. 
\textit{Data-driven discovery of coordinates and governing equations, PNAS, 116, No 45, pp. 22445—22451, 2019}


\bibitem{Elsner}
J. B. Elsner and A. Tsonis. \textit{Singular Spectrum Analysis, 1996.}

\bibitem{Fraser}
A. M. Fraser and H. L. Swinney. \textit{Independent coordinates for strange attractors from mutual information, Phys. Rev. A 33, pp. 1134 – Published February 1986.}

\bibitem{Gentry}
C. Gentry. \textit{Computing arbitrary functions of encrypted data, Communications of the ACM, 53~(2010), pp. 97--105.}


\bibitem{Jo_2020}

Hyeonta Jo and Hwija Sona and Hyung Ju Hwang and Se Young Jung, \textit{Analysis of COVID-19 spread in South Korea using the SIR model with time-dependent parameters and deep learning,  medRxiv preprint, 2020, https://doi.org/10.1101/2020.04.13.20063412}

\bibitem{Lorenz_1963}
E. N. Lorenz. \textit{Deterministic Non-Periodic flow, J. Atmos. Sci, 20~(1963), pp. 34.}

\bibitem{Malone_1955}
\textit{Malone, T. F.,
\emph{ Applications of Statistical Methods in Weather Prediction},
Proc Natl Acad Sci U S A, 41, pp.806-815, 1955.}

\bibitem{Vautard_1989}

\textit{Vautard, R. and M. Ghil,
\emph{ Singular spectrum analysis in nonlinear dynamics, with applications to paleoclimatic time series}, Physics D, 35, pp. 395–424, 1989. }

\bibitem{Richardson_1965}
\textit{Richardson, L. F.,
\emph{Weather prediction by numerical process. New York}, Dover Publications, 1965.}

\bibitem {Savitzky_1964}

\textit {Abraham. Savitzky and M. J. E. Golay,
Smoothing and Differentiation of Data by Simplified Least Squares Procedures. A. Savitzky and M. J. E. Golay, Analytical Chemistry, Vol 36, No.8, July 1964, pp.1627}

\bibitem{Schmid_2010}

\textit{Schmid, P., Dynamic mode decomposition of numerical and experimental data. Journal of Fluid Mechanics, Cambridge University Press (CUP), August 2010, vol 656 , pp. 5-28}

\bibitem {Mortari_2017}

\textit{Least Squares Solutions of Linear Differential Equations, Mortari, D. Least-Squares Solution of Linear Differential Equations. Mathematics 2017, 5, 48. }

\bibitem{Nekrutkin_2010}

\textit {V. Nekrutkin}, Perturbation expansions of signal subspaces for long signals , Statistics and Its Interface, 2010, pages = {297--319}
    

\bibitem {Burden_2011}

\textit{Burden, R. L., and Faires, J. D. (2011). Numerical analysis. Boston, Massachusetts: Brooks/Cole, Cengage Learning.}



\end{thebibliography}
